Quantifying the robustness of deep multispectral segmentation models against natural perturbations and data poisoning

In overhead image segmentation tasks, including additional spectral bands beyond the traditional RGB channels can improve model performance. However, it is still unclear how incorporating this additional data impacts model robustness to adversarial attacks and natural perturbations. For adversarial robustness, the additional information could improve the model's ability to distinguish malicious inputs, or simply provide new attack avenues and vulnerabilities. For natural perturbations, the additional information could better inform model decisions and weaken perturbation effects or have no significant influence at all. In this work, we seek to characterize the performance and robustness of a multispectral (RGB and near infrared) image segmentation model subjected to adversarial attacks and natural perturbations. While existing adversarial and natural robustness research has focused primarily on digital perturbations, we prioritize on creating realistic perturbations designed with physical world conditions in mind. For adversarial robustness, we focus on data poisoning attacks whereas for natural robustness, we focus on extending ImageNet-C common corruptions for fog and snow that coherently and self-consistently perturbs the input data. Overall, we find both RGB and multispectral models are vulnerable to data poisoning attacks regardless of input or fusion architectures and that while physically realizable natural perturbations still degrade model performance, the impact differs based on fusion architecture and input data.

==> tmp.tex <==

With the wealth of publicly available satellite imagery data and the development of large annotated satellite imagery datasets, deep learning models routinely achieve state-of-the-art performance in a number of important remote sensing applications, including land cover classification, agricultural monitoring, and disaster assessment. Typically, satellite sensors collect multispectral imagery, or imagery observed at wavelength bands beyond the traditional Red, Green, and Blue (RGB) bands found in natural imagery datasets. For many overhead imagery applications, spectral bands beyond the visible spectrum (e.g., near-infrared or short-wave infrared) are essential in distinguishing different surface materials or penetrating atmospheric haze. Deep learning models that leverage multispectral imagery are becoming increasingly common, and outperform RGB-only models in some applications (cite).

Over the past decade, there has been growing interest in understanding the robustness of deep learning models. To date, much of this research has focused on evaluating model performance on image classification tasks using benchmark RGB image datasets. As such, our understanding of model robustness for other tasks and data modalities remains incomplete. In this work, we make incremental progress towards this goal with an assessment of the robustness of deep image segmentation models applied to multispectral imagery, focusing on the combination of RGB and near-infrared (NIR) bands. 

For a given model, there are many possible ways to synthesize or fuse information from different inputs or data modalities. Models that combine data modalities at the input stage are sometimes called ``early fusion'' models (e.g., a 4-band image, or projecting 3D LiDAR data onto an RGB image). In contrast, a model that processes the different data modalities separately and combines them after feature extraction or in the final layer before classification would be called a ``late fusion'' model. In this work, we are specifically interested in quantifying the robustness of different fusion approaches. To this end, we explore different combinations of input bands (NIR, RGB, RGB+NIR) and architectures (early vs. late fusion) to better understand how each of these variables affects the model's overall robustness, and explore any potential trade-offs with model performance. 

Since the introduction of adversarial examples (cite), researchers have tried to better understand model properties connected to robustness. Robustness refers to a model's ability to maintain performance under various input shifts, including natural shifts (e.g., weather, environment) and adversarial shifts (e.g., attacks or digital perturbations). While many advancements have emerged in the field of robustness, deep learning models remain vulnerable to various attacks and distribution shifts. In this work, we consider both adversarial robustness and natural robustness for segmentation models, with an emphasis on perturbations that are physically meaningful for multispectral imagery.

While a multitude of adversarial attacks exist in the literature, digital adversarial examples remain the most well-studied attack type. Adversarial examples have been applied to many visual perception tasks, including image segmentation\cite{xie_adversarial_2017} \cite{vo_multiclass_2022} \cite{gu_segpgd_2022} \cite{yin_adversarial_2022} \cite{arnab_robustness_nodate}. However, adversarial example attacks often have unrealistic access requirements and their real-world feasibility is limited. In this work, we focus on data poisoning, wherein adversaries inject malicious data into the training data to cause erroneous classifications or backdoor access during test time. In a field where it is common for researchers to download datasets from a variety of unregulated sources, data poisoning is one of the more practical attacks in the literature. With the rise in the number of commercial companies that both collect satellite imagery and generate data products, data poisoning will continue to be relevant in satellite imagery applications. To our knowledge, this is the first assessment of data poisoning attacks on multispectral imagery in image segmentation models.

For a more comprehensive picture of model robustness, we also consider natural robustness. Natural robustness is well studied in the context of RGB imagery, with published libraries for domain adaptation tests, natural perturbation datasets, and data augmentation approaches that reflect real-world variations. However, there aren't established processes to extend these natural perturbations beyond the visible spectrum in a way that is physically consistent. In this work, we develop an approach for physically realistic perturbations that can be applied to multispectral imagery. We then quantify the robustness of the segmentation models, assessing the relative accuracy and robustness of different fusion approaches compared to an RGB model baseline.

%Moreover, robustness papers typically only consider digital perturbations, and physically-realizable applications are limited, especially in the context of different data modalities. 







%In overhead imagery applications, research has shown that including additional spectral bands can improve image segmentation performance \cite{zhang_deep_2021}. However, it is still unclear if this additional information also introduces new vulnerabilities.
%With more affordable sensors on the market and the rise in available data, deep learning models have been developed for many different data modalities. A multimodal model is a model designed to leverage multiple types of data to improve model performance. These models may combine similar data modalities, like RGB and thermal infrared imagery, or combine disparate data streams, like LiDAR, audio, or text. Multimodal models have been applied in various applications, including autonomous driving, image captioning, and medical image-text diagnostics, and can sometimes achieve better performance than a unimodal model (cite).
%As research has progressed, . Adversarial robustness aims to assess how resilient a model is when attacked, while natural robustness tries to gauge a model's ability to withstand real-world perturbations and changes. 
%In this work, we address some of these issues by comparing adversarial and physically-realizable robustness for models in a less studied domain, focusing on image segmentation models applied to overhead multispectral imagery. 

%With more affordable sensors on the market and the rise in available data, deep learning models have been developed for many different data modalities, including images, text, audio, LiDAR.

% We help answer whether extra channels leads to a larger attack space or leads to extra protection to a model.
%Adversarial robustness is part of adversarial machine learning, a means to better understand the overall vulnerabilities that exist in machine learning model.
%To investigate the vulnerabilities and understand multimodal segmentation model robustness, we do the following: investigate adversarial attacks and natural perturbation effects on models; compare these effects on single vs multimodal models; and compare various fusion types for multimodal models.

Over the past decade, there has been growing interest in understanding the robustness of deep learning models. To date, much of this research has focused on evaluating model performance on image classification tasks using benchmark RGB image datasets. As such, our understanding of model robustness for other tasks and data modalities remains incomplete.
% with the wealth of satellite data, more bands are available
% multspectral models exist and have shown improved performance
% we don't know the robustness of these kinds of models and data

% what is model robustness
As research has progressed, two distinct but related measures of robustness have developed: adversarial robustness and natural robustness. Adversarial robustness aims to assess how resilient a model is when attacked, while natural robustness tries to gauge a model's ability to withstand real-world perturbations and changes. While many advancements have emerged in the field of robustness, deep learning models remain vulnerable to various attacks and perturbations.  Moreover, natural robustness papers typically only consider digital perturbations, and physically-realizable applications are limited, especially in the context of different data modalities. 

In this work, we address some of these issues by comparing adversarial and physically-realizable robustness for models in a less studied domain, focusing on image segmentation models applied to overhead multispectral imagery. For overhead imagery applications, research has shown that including additional spectral bands can improve image segmentation performance (cite). However, it is still unclear if this additional information also introduces new vulnerabilities. Here, we explore different combinations of input bands (NIR, RGB, RGB+NIR) and architectures (early vs. late fusion) to better understand how each of these variables affects the model's overall robustness, and explore any potential trade-offs with model performance. 

For a more comprehensive picture of model robustness beyond typical adversarial example attacks, we test the effectiveness of both data poisoning attacks and physically realizable digital perturbations. [Sentence introducing how natural robustness solutions don't easily extend to new data modalities] [we develop realistic corruptions for multispectral data] 

% We help answer whether extra channels leads to a larger attack space or leads to extra protection to a model.
%Adversarial robustness is part of adversarial machine learning, a means to better understand the overall vulnerabilities that exist in machine learning model.
%To investigate the vulnerabilities and understand multimodal segmentation model robustness, we do the following: investigate adversarial attacks and natural perturbation effects on models; compare these effects on single vs multimodal models; and compare various fusion types for multimodal models.



\subsection{Related Work}

\subsubsection{Multimodal Models and Fusion Methods}

In XXX, the authors compared different fusion approaches for RGB and thermal natural imagery, and assessed model robustness to digital adversarial attacks in the context of image classification. This work builds upon XXX, but differs in a few key ways: First, we move from image classification to image segmentation, which adds complexity, and is a less studied task. Second, we move from natural imagery to overhead imagery, increasing the domain shift from benchmark research. Third, we expand the adversarial attack space considered by including data poisoning and physically-realizable attacks.


\subsubsection{Adversarial and Natural Robustness}

In this work, we focus on model robustness to both digital perturbations and data poisoning attacks. In \cite{li_hidden_2021}, the authors demonstrate the efficacy of data poisoning attacks to image segmentation models on RGB imagery. We extend the assessment of adversarial resiliency from \cite{li_hidden_2021} to include both unimodal and multimodal segmentation models. We are particularly interested in understanding the balance between performance and robustness in multispectral segmentation models compared to traditional RGB models, and the context in which vulnerabilities are improved or worsened.
% probably need to cite: DAG attack - adversarial examples, overhead imagery

To do: think about how to do this separation. some object detection \cite{yang_defending_2021} \cite{wang_adversarial_2022} \cite{du_adversarial_2021} and semantic segmentation \cite{yu_investigating_2020}

Robustness paper that looks at it from segmentation model perspective \cite{kamann_benchmarking_2020}.

% look for citations on common corruptions? for image segmentation? or overhead imagery, but only RGB

% While there is overlap between adversarial and natural robustness research, adversarial robustness research tends to focus on identifying vulnerabilities in deep learning models. Attack techniques in the literature include adversarial examples, membership inference, model stealing, and data poisoning, as well as methods to defend a model such as adversarial training, data distribution monitoring, and data sanitization. Natural robustness research tends to focus on making models more resilient to input changes that are likely to occur in the real world. Published approaches include natural perturbation datasets and creating domain adaptation tests while also developing methods to promote natural robustness such as data augmentation, out of distribution data detection, and improving data collection to ensure it reflects real-world variations and conditions. 

